Neural-PIL: Neural Pre-Integrated Lighting for Reflectance Decomposition

Decomposing a scene into its shape, reflectance and illumination is a fundamental problem in computer vision and graphics. Neural approaches such as NeRF have achieved remarkable success in view synthesis, but do not explicitly perform decomposition and instead operate exclusively on radiance (the product of reflectance and illumination). Extensions to NeRF, such as NeRD, can perform decomposition but struggle to accurately recover detailed illumination, thereby significantly limiting realism. We propose a novel reflectance decomposition network that can estimate shape, BRDF, and per-image illumination given a set of object images captured under varying illumination. Our key technique is a novel illumination integration network called Neural-PIL that replaces a costly illumination integral operation in the rendering with a simple network query. In addition, we also learn deep low-dimensional priors on BRDF and illumination representations using novel smooth manifold auto-encoders. Our decompositions can result in considerably better BRDF and light estimates enabling more accurate novel view-synthesis and relighting compared to prior art. Project page: https://markboss.me/publication/2021-neural-pil/

==> figures/architecture/brdf.tex <==
\begin{tikzpicture}[node distance=0.15cm]%

\node(gtBrdf) {$\vect{b}$};

% Encoder
\node[rounded corners=2pt, draw=mteal, fill=mteallight, line width=1.5pt, inner sep=0.1cm, below right=0.5cm of gtBrdf] (Enc) {$\text{E}$};

% Embedding
\node[below=of Enc] (embd) {$\vect{z}$};

% Direct z reconstruction
\node[rounded corners=2pt, draw=morange, fill=morangelight, line width=1.5pt, inner sep=0.1cm, below=of embd] (DecZ) {$\text{G}$};
\node[below=of DecZ] (zBrdf) {$\vect{\hat{b}}$};
\node[circle, draw, inner sep=0.5mm] (Lr) at (zBrdf -| gtBrdf) {$\mathcal{L}_r$}; % Loss function reconstruction

% Reconstruction loss
\draw[draw=mred,thick,dotted] ($(gtBrdf.north -| Lr.west)+(-0.1,0.1)$)  rectangle ($(Lr.south -| DecZ.east)+(0.1,-0.1)$);
\node[below=0.45cm of $(Lr)!0.5!(zBrdf)$, font=\scriptsize\linespread{0.8}\selectfont, text width=1.5cm, align=center] (supervisedLabel) {Supervised Reconstruction};

% Split Embedding
\coordinate[right=1cm of embd] (interpolEmbdHeight);
\node[above=of interpolEmbdHeight] (embd1) {$\vect{z_i}$};
\node[below=of interpolEmbdHeight] (embd2) {$\vect{z_j}$};

% Interpolation alpha
\node (alpha) at (gtBrdf -| embd1) {$\alpha$};
\node[draw=black, right=0.5cm of $(embd1)!0.5!(embd2)$] (interpol) {$\vect{z}_{i \rightarrow j}(\alpha)$};

% Decoded again
\node[rounded corners=2pt, draw=morange, fill=morangelight, line width=1.5pt, inner sep=0.1cm, right=of interpol] (DecZij) {$\text{G}$};
\node[right=of DecZij] (zijBrdf) {$\vect{\hat{b}}_{i \rightarrow j}(\alpha)$};

\draw[draw=mblue,thick,dotted] ($(embd1.north west)+(-0.1,0.1)$)  rectangle ($(embd2.south -| zijBrdf.south east)+(0.1,-0.1)$);
\node[below=0.45cm of $(embd2.south)!0.5!(zijBrdf)$, font=\scriptsize\linespread{0.8}\selectfont, text width=1.5cm, align=center] {Interpolation};

% Cyclic loss
\node[rounded corners=2pt, draw=mteal, fill=mteallight, line width=1.5pt, inner sep=0.1cm, above=0.6cm of zijBrdf] (CycleEnc)  {$\text{E}$};
\node[above=of CycleEnc] (cycleEmbd) {$\vect{\hat{z}}_{i \rightarrow j}(\alpha)$};
\node[circle, draw, inner sep=0.5mm, left=of cycleEmbd] (Lc) {$\mathcal{L}_c$}; % Loss function cyclic

% Smoothness loss
\node[circle, draw, inner sep=0.5mm] (Ls) at (Lc -| interpol) {$\mathcal{L}_s$}; % Loss function smoothness

\node[rounded corners=2pt, draw=mpurple, fill=mpurplelight, line width=1.5pt, inner sep=0.1cm] (Discrim) at (zBrdf -| zijBrdf) {$\text{D}$};
\node[circle, draw, inner sep=0.5mm, right=of Discrim] (La)  {$\mathcal{L}_a$}; % Loss function adversarial

\draw[draw=mgreen,thick,dotted] ($(Ls.north -| alpha.west)+(-0.3,0.1)$)  rectangle ($(La.south east)+(0.2,-0.2)$);
\coordinate (centerUnsupervised) at ($(embd2.west)!0.5!(La.east)$);
\node[font=\scriptsize\linespread{0.8}\selectfont, text width=1.5cm, align=center] at (supervisedLabel -| centerUnsupervised) {Unsupervised Reconstruction};

% Lines
\draw[->] 
    (gtBrdf) edge (Enc)
    (Enc) edge (embd)
    (embd) edge (DecZ)
    (DecZ) edge (zBrdf)
    (gtBrdf) edge (Lr)
    (zBrdf) edge (Lr)
    (interpol) edge (DecZij)
    (DecZij) edge (zijBrdf)
    (zijBrdf) edge (Discrim)
    (Discrim) edge (La)
    (zijBrdf) edge (CycleEnc)
    (CycleEnc) edge (cycleEmbd)
    (cycleEmbd) edge (Lc);
    
\draw[->] (interpol) to [out=60, in=270] (Lc);
\draw[->] (alpha) to [out=0, in=180] (Ls);
\draw[->] (alpha) to [out=0, in=110] (interpol);

\draw[->] (zijBrdf) to [out=110, in=270] (Ls);

\draw[->] (embd) to [out=0, in=180] (embd1);
\draw[->] (embd) to [out=0, in=180] (embd2);

\draw[->] (embd1) to [out=350, in=170] (interpol);
\draw[->] (embd2) to [out=10, in=190] (interpol);

\end{tikzpicture}

==> figures/architecture/fine_simple.tex <==
\begin{tikzpicture}[
    node distance=0.15cm,
    layer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.2cm, rounded corners=1pt},
    textlayer/.style={draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    encoder/.style={isosceles triangle,isosceles triangle apex angle=60,shape border rotate=0,anchor=apex,draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    decoder/.style={isosceles triangle,isosceles triangle apex angle=60,shape border rotate=180,anchor=apex,draw=#1, fill=#1!20, line width=1.5pt, inner sep=0.1cm, rounded corners=1pt},
    label/.style={font=\scriptsize, text width=1.2cm, align=center},
    fourier/.pic={%
        \node (#1){
            \begin{tikzpicture}[remember picture]%
                \draw[line width=0.75pt] (0,0) circle (6pt);%
                \draw[line width=0.75pt] (-6pt,0.0) sin (-3pt,2pt) cos (0,0) sin (3pt,-2pt) cos (6pt,0);%
            \end{tikzpicture}
        };
    }
]%
% cblue3 main net
% cblue5 conditional
% cdiv15 BRDF ae
% corange3 illumination ae
    
\node[label] (input) {Position $\vect{x}$};

\pic[right=of input] {fourier=fourier};

% Main Network
\node[textlayer={white}, font=\tiny, right=0.225cm of fourier] (main_mlp1) {\rotatebox{90}{Linear}};
\node[textlayer={white}, font=\tiny, right=0.075cm of main_mlp1] (main_relu1) {\rotatebox{90}{ReLU}};
\node[right=0.075cm of main_relu1, font=\tiny] (ellipse) {\rotatebox{90}{\ldots}};
\node[textlayer={white}, font=\tiny, right=0.075cm of ellipse] (main_mlp2) {\rotatebox{90}{Linear}};

% Background and label
\begin{scope}[on background layer]
    \draw[layer={cblue3}, rounded corners=1pt,line width=0.75pt] ($(main_mlp1.north west)+(-0.075,0.075)$)  rectangle ($(main_mlp2.south east)+(0.075,-0.075)$);
\end{scope}
\node[above=of $(main_mlp1.north)!0.5!(main_mlp2.north)$, label, text width=1.5cm] {Main Network};

% BRDF Decoder
\node[textlayer={cdiv15}, right=0.3cm of main_mlp2, draw=white, fill=white, text=white] (brdf_network) {\rotatebox{90}{\tiny BRDF SMAE}};

% Renderer
\node[textlayer={cblue5}, right=0.3cm of brdf_network] (renderer) {\rotatebox{90}{\tiny Renderer}};

% Remaining inputs
\node[label, below=of input |- main_mlp1.south] (view_direction) {View Direction $\vect{\omega}_o$};
\node[label, below=of view_direction] (illumination_embedding) {Illumination};

% Sigma extraction
\coordinate (between_network_renderer) at ($(main_mlp2)!0.5!(brdf_network)$);
\node[label, above=of between_network_renderer |- brdf_network.north] (density) {Density $\sigma$};
\node[label, right=of density] (normal) {Normal $\vect{n}$};
\draw[->] (density) -- (normal) node [midway, above] {\scriptsize $\nabla \sigma_x$};

% Get light direction
% \node[label] (reflect) at (normal |- view_direction) {Reflect};
% \node[label, below=of reflect] (light_direction) {Light Direction $\vect{\omega}_i$};

% PIL
% \node[textlayer={corange3}, right=0.5cm of illumination_embedding] (pil) {\tiny Neural-PIL};

% Output
\node[label, right=0.5cm of renderer] (output) {Color $\vect{c}$};

% Draw connection

% Main connections
\draw[->, shorten >=-0.1cm] (input) -- (fourier);
\draw[->, shorten <=-0.1cm, shorten >=0.075cm] (fourier) -- (main_mlp1);
\draw[->, shorten <=0.075cm] (main_mlp2) -- (renderer);
% \draw[->] (brdf_network) -- (renderer);
\draw[->, shorten >=-0.2cm] (renderer) -- (output);

% Density, normal, reflect
\draw[->] (between_network_renderer) -- (density);
% \draw[->] (normal) -- (reflect);
% \draw[->,shorten >=-0.2cm] (view_direction) -- (reflect);
% \draw[->] (reflect) -- (light_direction);
\draw[->] (normal) edge[out=270, in=90] (renderer);

% PIL network
\draw[->] (illumination_embedding) edge[out=0, in=270] (renderer);
\draw[->] (view_direction) edge[out=0, in=270] (renderer);
% \draw[->] (pil) edge[out=0, in=270] (renderer);
% \draw[->] (light_direction) edge[out=180, in=90] (pil);
% \draw[->] (brdf_network) edge[out=270, in=90] (pil);

    
\end{tikzpicture}

==> figures/architecture/illumination.tex <==
\newcommand\padding{0.08cm}
\newcommand\outline{0.2pt}
\newcommand\layerwidth{0.05cm}
\newcommand\layers{3}
\newcommand\networkwidth{2*\padding + \layers * 2 * \layerwidth * 2 - \layerwidth}
\newcommand\nodeheight{0.5cm}

\begin{tikzpicture}[node distance=0.15cm]%

\node(spherical_input) {$\theta, \phi$};

\node[rounded corners=2pt, draw=mblue, fill=mbluelight, line width=1.5pt, inner sep=0.1cm, minimum width=0.4cm, minimum height=1.2cm, right=of spherical_input] (mlp1) {};
\node[rounded corners=2pt, draw=mblue, fill=mbluelight, line width=1.5pt, inner sep=0.1cm, minimum width=0.4cm, minimum height=1.2cm, right=of mlp1] (mlp2) {};
\node[rounded corners=2pt, draw=mblue, fill=mbluelight, line width=1.5pt, inner sep=0.1cm, minimum width=0.4cm, minimum height=1.2cm, right=of mlp2] (mlp3) {};
\node[rounded corners=2pt, draw=mblue, fill=mbluelight, line width=1.5pt, inner sep=0.1cm, minimum width=0.4cm, minimum height=1.2cm, right=of mlp3] (mlp4) {};

\node[right=of mlp4] (hadamard) {$\odot$};
\node[rounded corners=2pt, draw=mgreen, fill=mgreenlight, line width=1.5pt, inner sep=0.1cm, minimum width=0.4cm, minimum height=1.2cm, right=of hadamard] (mlp_rough) {};

% hadamard main join
\node[
        rounded corners=2pt, 
        rectangle split,
        rectangle split horizontal,
        rectangle split parts=2,
        rectangle split part fill={mbluelight,mgreenlight},
        line width=0pt, inner sep=0.09cm, 
        text width=0.02cm, minimum height=1.15cm,
        right=of mlp_rough
    ] (hadamard_mlp) {\nodepart{two}};
% Try to split color the border
\begin{scope}[on background layer]
\node[
        rounded corners=2pt, 
        rectangle split,
        rectangle split horizontal,
        rectangle split parts=2,
        rectangle split part fill={mblue,mgreen},
        line width=0pt, inner sep=0.118cm, 
        text width=0.02cm, minimum height=1.26cm,
    ] (hadamard_mlp_border) at (hadamard_mlp) {\nodepart{two}};
\end{scope}    
    

\node[rounded corners=2pt, draw=mblue, fill=mbluelight, line width=1.5pt, inner sep=0.1cm, minimum width=0.4cm, minimum height=1.2cm, right=of hadamard_mlp] (mlp5) {};

\node [isosceles triangle,
      isosceles triangle stretches,
      rotate=90, yshift=-0.2cm, xshift=0.15cm, 
      inner sep=0cm, minimum width=0.4cm, minimum height=0.8cm, 
      draw=mgrayblue, fill=mgraybluelight, line width=1.5pt, 
      above=of mlp1] (cnn1) {};
\node [isosceles triangle,
      isosceles triangle stretches,
      rotate=90, yshift=-0.2cm, xshift=0.15cm, 
      inner sep=0cm, minimum width=0.4cm, minimum height=0.8cm, 
      draw=mgrayblue, fill=mgraybluelight, line width=1.5pt, 
      above=of mlp2] (cnn2) {};
\node [isosceles triangle,
      isosceles triangle stretches,
      rotate=90, yshift=-0.2cm, xshift=0.15cm, 
      inner sep=0cm, minimum width=0.4cm, minimum height=0.8cm, 
      draw=mgrayblue, fill=mgraybluelight, line width=1.5pt, 
      above=of mlp3] (cnn3) {};
\node [isosceles triangle,
      isosceles triangle stretches,
      rotate=90, yshift=-0.2cm, xshift=0.15cm, 
      inner sep=0cm, minimum width=0.4cm, minimum height=0.8cm, 
      draw=mgrayblue, fill=mgraybluelight, line width=1.5pt, 
      above=of mlp4] (cnn4) {};
\node [isosceles triangle,
      isosceles triangle stretches,
      rotate=90, yshift=-0.2cm, xshift=0.15cm, 
      inner sep=0cm, minimum width=0.4cm, minimum height=0.8cm, 
      draw=mgrayblue, fill=mgraybluelight, line width=1.5pt, 
      above=of mlp5] (cnn5) {};
      
\node[above left=of cnn1.north, text width=1.4cm, font=\tiny\linespread{0.8}\selectfont] {1D CNN Weight \& Bias Generator};

\node[above=of cnn1.east -| spherical_input] (embedding_input) {$\vect{z}$};


\node[below=of mlp1.south -| spherical_input] (roughness_input) {$b_r$};

\coordinate[right=1cm of mlp5] (mlp_output);
\node[above=0.01cm of mlp_output] (mlp_sampling) {\includegraphics[width=1.75cm,trim=0 150 0 0,clip]{figures/architecture/NeRDSampleR0.png}};

\node[below=0.1cm of mlp_output] (mlp_sampling_r5) {\includegraphics[width=1.75cm,trim=0 150 0 0,clip]{figures/architecture/NeRDSampleR05.png}};

\node[font=\tiny\linespread{0.8}\selectfont, text width=1.4cm, yshift=-0.1cm, align=center] at (mlp_output) {Effect of varying roughness};


\draw[->, to path={-| (\tikztotarget)}]
  (embedding_input) edge (cnn1)
  (embedding_input) edge (cnn2)
  (embedding_input) edge (cnn3)
  (embedding_input) edge (cnn4)
  (embedding_input) edge (cnn5)
  (roughness_input) edge (mlp_rough);
  
\draw
    (spherical_input) edge(mlp1)
    (mlp1) edge(mlp2)
    (mlp2) edge(mlp3)
    (mlp3) edge(mlp4)
    (hadamard_mlp_border) edge(mlp5);
  

% \filldraw[rounded corners=1pt, draw=mblue, fill=mbluelight, line width=\outline, inner sep=0pt, right=of spherical_input] rectangle (\networkwidth,\nodeheight);


\end{tikzpicture}


%\filldraw[draw=#1, fill=#1!20,line width=\outline, inner sep=0pt] (\padding+6*\layerwidth,\padding+2*\layerwidth) rectangle (\padding+7*\layerwidth,\nodeheight-\padding-2*\layerwidth);

==> figures/nerf_comparison/comparison.tex <==
\scriptsize%
\renewcommand{\arraystretch}{0.6}%
\setlength{\tabcolsep}{0pt}%
\begin{tabular}{@{}%
>{\centering\arraybackslash}m{41pt}% GT
>{\centering\arraybackslash}m{41pt}% NeRF
>{\centering\arraybackslash}m{41pt}% Ours
@{\hskip 5mm}%
>{\centering\arraybackslash}m{41pt}% GT
>{\centering\arraybackslash}m{41pt}% NeRF
>{\centering\arraybackslash}m{41pt}% Ours
@{\hskip 5mm}%
>{\centering\arraybackslash}m{41pt}% GT
>{\centering\arraybackslash}m{41pt}% NeRF
>{\centering\arraybackslash}m{41pt}% Ours
@{}}%
GT & NeRF & Ours & GT & NeRF & Ours & GT & NeRF & Ours \\ \vspace{1mm}
\includegraphics[width=41pt]{figures/nerf_comparison/gt/1_gt_rgb.png} & %
\includegraphics[width=41pt]{figures/nerf_comparison/nerf/001_rgb_0.png}&
\includegraphics[width=41pt]{figures/nerf_comparison/ours/1_fine_rgb.png}& 
\includegraphics[width=41pt]{figures/nerf_comparison/gt/2_gt_rgb.png} & %
\includegraphics[width=41pt]{figures/nerf_comparison/nerf/002_rgb_0.png}&
\includegraphics[width=41pt]{figures/nerf_comparison/ours/2_fine_rgb.png}& 
\includegraphics[width=41pt]{figures/nerf_comparison/gt/5_gt_rgb.png} & %
\includegraphics[width=41pt]{figures/nerf_comparison/nerf/005_rgb_0.png}&
\includegraphics[width=41pt]{figures/nerf_comparison/ours/5_fine_rgb.png}
\end{tabular}

==> figures/real_world_example/comparison.tex <==
\normalsize%
\renewcommand{\arraystretch}{0.6}%
\setlength{\tabcolsep}{0pt}%
\begin{tabular}{@{}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}>{\centering\arraybackslash}m{33pt}@{}}%
%\toprule%
\tiny Diffuse&\tiny Specular&\tiny Roughness&\tiny Normal&\tiny GT&\tiny Re{-}render - Illum 0&\tiny Illum 1&\tiny View + Illum 1&\tiny View + Illum 2&\tiny View + Illum 0\\%
\midrule%
\includegraphics[width=33pt,trim=0 0 125 80, clip]{figures/real_world_example/gnome/4_fine_diffuse.jpg}&\includegraphics[width=33pt,trim=0 0 125 80, clip]{figures/real_world_example/gnome/4_fine_specular.jpg}&\includegraphics[width=33pt,trim=0 0 125 80, clip]{figures/real_world_example/gnome/4_fine_roughness.jpg}&\includegraphics[width=33pt,trim=0 0 125 80,clip]{figures/real_world_example/gnome/4_fine_normal.jpg}&\includegraphics[width=33pt,trim=0 0 125 80,clip]{figures/real_world_example/gnome/4_gt_rgb.jpg}&\includegraphics[width=33pt,trim=0 0 125 80,clip]{figures/real_world_example/gnome/4_48_rgb.jpg}&\includegraphics[width=33pt,trim=0 0 125 80,clip]{figures/real_world_example/gnome/4_32_rgb.jpg}&\includegraphics[width=33pt,trim=0 0 125 80,clip]{figures/real_world_example/gnome/3_32_rgb.jpg}&\includegraphics[width=33pt,trim=0 0 125 80,clip]{figures/real_world_example/gnome/3_0_rgb.jpg}&\includegraphics[width=33pt,trim=0 0 125 80,clip]{figures/real_world_example/gnome/3_48_rgb.jpg}\\\midrule %
\tiny GT&\tiny Re{-}render - Illum 0&\tiny Illum 1&\tiny View + Illum 1&\tiny View + Illum 0& \tiny GT&\tiny Re{-}render - Illum 0&\tiny Illum 1&\tiny View + Illum 1& \tiny View + Illum 0\\\midrule%
\includegraphics[width=33pt]{figures/real_world_example/cape/IMG_5993.jpg}&\includegraphics[width=33pt]{figures/real_world_example/cape/112_render.jpg}&\includegraphics[width=33pt]{figures/real_world_example/cape/112_r1.jpg}&\includegraphics[width=33pt]{figures/real_world_example/cape/48_r1.jpg}&\includegraphics[width=33pt]{figures/real_world_example/cape/48_render.jpg}& %
% \includegraphics[width=33pt,trim=55 10 55 0,clip]{figures/real_world_example/duckqueen/IMG_1207.jpg}&\includegraphics[width=33pt,trim=145 40 145 0,clip]{figures/real_world_example/duckqueen/144_r0.jpg}&\includegraphics[width=33pt,trim=145 40 145 0,clip]{figures/real_world_example/duckqueen/144_r1.jpg}&\includegraphics[width=33pt,trim=195 40 95 0,clip]{figures/real_world_example/duckqueen/96_r1.jpg}&\includegraphics[width=33pt,trim=195 40 95 0,clip]{figures/real_world_example/duckqueen/96_r0.jpg}& %
% \includegraphics[width=33pt,trim=35 10 35 0,clip]{figures/real_world_example/blowtorch/_DSC1587.jpg}&\includegraphics[width=33pt,trim=145 40 145 0,clip]{figures/real_world_example/blowtorch/80_org.jpg}&\includegraphics[width=33pt,trim=145 40 145 0,clip]{figures/real_world_example/blowtorch/80_r1.jpg}&\includegraphics[width=33pt,trim=195 40 95 0,clip]{figures/real_world_example/blowtorch/32_r1.jpg}&\includegraphics[width=33pt,trim=195 40 95 0,clip]{figures/real_world_example/blowtorch/32_org.jpg}& %
\includegraphics[width=33pt,trim=55 15 63 0,clip]{figures/real_world_example/motherchild/IMG_1004.jpg}&\includegraphics[width=33pt,trim=55 15 63 0,clip]{figures/real_world_example/motherchild/64_org.jpg}&\includegraphics[width=33pt,trim=55 15 63 0,clip]{figures/real_world_example/motherchild/64_r1.jpg}&\includegraphics[width=33pt,trim=55 15 63 0,clip]{figures/real_world_example/motherchild/96_r1.jpg}&\includegraphics[width=33pt,trim=55 15 63 0,clip]{figures/real_world_example/motherchild/96_org.jpg}%
\\%
%&&&&\scriptsize MSE: 0.0248&&\\%\bottomrule%
%
\end{tabular}%


==> figures/table_illumination.tex <==
\scriptsize%

\setlength{\tabcolsep}{2pt}%
\begin{tabular}{lccC}%
    \toprule%
    \multicolumn{1}{c}{Method} & Shape & BRDF & \text{[MALE\textdownarrow]} \\%
    \midrule%
    \scriptsize Li \etal & \cmark & \cmark & \text{0.6240} \\ 
    %\scriptsize Weber \etal~\cite{weber2018} & known & not optimized & \text{---} \\
    \scriptsize NeRD & \cmark & \cmark &  \text{0.6066}          \\%
    \scriptsize Ours & \cmark  & \cmark &   \text{---} \\\bottomrule%
    %
\end{tabular}%

% NeRD-II
% Scene: Globe
% Diffuse         Specular        Roughness       Environment
% 0.689159        0.015210        0.006347        0.243203

% NeRD
% Scene: Globe
% Diffuse Specular        Roughness       Environment
% 0.014539        0.005054        0.077825        0.737097
% Scene: Wreck
% Diffuse Specular        Roughness       Environment
% 0.013085        0.002251        0.008537        0.650299
% Scene: Chair
% Diffuse Specular        Roughness       Environment
% 0.017636        0.001066        0.010017        0.432639
% Overall: ['Globe', 'Wreck', 'Chair']
% Diffuse Specular        Roughness       Environment
% 0.015087        0.002790        0.032127        0.606678

% Li
% Scene: Globe
% Diffuse Roughness       Environment
% 0.733816        0.031004        0.602380
% Scene: Wreck
% Diffuse Roughness       Environment
% 0.819685        0.014023        0.639668
% Scene: Chair
% Diffuse Roughness       Environment
% 0.797146        0.012133        0.630079
% Overall: ['Globe', 'Wreck', 'Chair']
% Diffuse Roughness       Environment
% 0.783549        0.019053        0.624042

==> figures/table_novel.tex <==
\scriptsize%

\setlength{\tabcolsep}{2pt}%
\begin{tabular}{llCCCC}%
    \toprule%
                                            & & \multicolumn{2}{c}{Fixed Illumination} & \multicolumn{2}{c}{Varying Illumination} \\
    \cmidrule(l){3-4} \cmidrule(l){5-6}
    & \multicolumn{1}{c}{Method} & \multicolumn{1}{c}{PSNR\textuparrow} & \multicolumn{1}{c}{SSIM\textuparrow} & \multicolumn{1}{c}{PSNR\textuparrow} & \multicolumn{1}{c}{SSIM\textuparrow}\\%
    \midrule%
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\scriptsize Synthetic}}} & \scriptsize NeRF %
    & \mathbf{31.3966}       & 0.9280   % Fixed Syn
    & 21.2860                & 0.9108\\% Var Syn
    & \scriptsize NeRD                        %
    & 28.7277             & 0.9381      % Fixed Syn           
    & 22.8390             & 0.9160\\
    & \scriptsize Ours                        %
    & 27.1061             & \mathbf{0.9402}                 % Fixed Syn           
    & \mathbf{28.8926}  & \mathbf{0.9574} \\\midrule% Var Syn
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\scriptsize Real}}} & \scriptsize NeRF  %
    & 23.1013             & 0.8936   % Fixed RW     
    & 22.2083                & 0.8972 \\% Var RW
    & \scriptsize NeRD          %               
    & 25.4678             & 0.8517       %Fixed RW         
    & 25.5525                & 0.9415 \\
    & \scriptsize Ours          %               
    & \mathbf{25.4855}             & \mathbf{0.9162}      %Fixed RW         
    & \mathbf{27.4254}               & \mathbf{0.9507} \\\bottomrule% Var RW
    %
\end{tabular}%

% NeRD-ii fixed synthetic
% Scene: Chair
% MSE      PSNR    SSIM
% 0.001180         29.448725       0.962094
% Synthetic nerf data
% Scene: Lego
% MSE      PSNR    SSIM
% 0.002152         26.725717       0.947572
% Synthetic nerf data
% Scene: Ship
% MSE      PSNR    SSIM
% 0.003166         25.143879       0.911110
% Overall: ['Chair', 'Lego', 'Ship']
% MSE      PSNR    SSIM
% 0.002166         27.106107       0.940259

% NeRD-ii varyin synthetic
% Scene: Globe
% MSE      PSNR    SSIM
% 0.003464         24.745599       0.920008
% Synthetic non nerf data
% Scene: Car
% MSE      PSNR    SSIM
% 0.001085         30.125778       0.971845
% Synthetic non nerf data
% Scene: Chair
% MSE      PSNR    SSIM
% 0.000753         31.806711       0.980645
% Overall: ['Globe', 'Car', 'Chair']
% MSE      PSNR    SSIM
% 0.001767         28.892696       0.957499


% NeRD-ii real fixed
% RW data
% Scene: Cape
% MSE      PSNR    SSIM
% 0.005061         23.625423       0.884584
% RW data
% /graphics/projects2/data/boss/Nerd-wdDataset/RealWorld/ethiopianHead/images_8
% ['DSC_0007', 'DSC_0023', 'DSC_0039', 'DSC_0055', 'DSC_0072']
% Scene: Head
% MSE      PSNR    SSIM
% 0.002324         27.345726       0.947840
% Overall: ['Cape', 'Head']
% MSE      PSNR    SSIM
% 0.003693         25.485575       0.916212

% Real varying
% Scene: Gnome
% MSE      PSNR    SSIM
% 0.002753         25.942879       0.927598
% RW data
% /graphics/projects2/data/boss/Nerd-wdDataset/RealWorld/mother_child-photogrammetry/images_8
% ['IMG_0936', 'IMG_0952', 'IMG_0969', 'IMG_0987', 'IMG_1004', 'IMG_1020', 'IMG_1039']
% Scene: MotherChild
% MSE      PSNR    SSIM
% 0.001398         28.907953       0.973884
% Overall: ['Gnome', 'MotherChild']
% MSE      PSNR    SSIM
% 0.002076         27.425416       0.950741

==> sections/checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Will be made available upon acceptance}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

